Learning Background Prompts to Discover Implicit Knowledge for Open Vocabulary Object Detection

Open vocabulary object detection (OVD) aims at seeking an optimal object detector capable of recognizing objects from both base and novel categories. Recent advances leverage knowledge distillation to transfer insightful knowledge from pre-trained large-scale vision-language models to the task of object detection, significantly generalizing the powerful capabilities of the detector to identify more unknown object categories. However, these methods face significant challenges in background interpretation and model overfitting and thus often result in the loss of crucial background knowledge, giving rise to sub-optimal inference performance of the detector. To mitigate these issues, we present a novel OVD framework termed LBP to propose learning background prompts to harness explored implicit background knowledge, thus enhancing the detection performance w.r.t. base and novel categories. Specifically, we devise three modules: Background Category-specific Prompt, Background Object Discovery, and Inference Probability Rectification, to empower the detector to discover, represent, and leverage implicit object knowledge explored from background proposals. Evaluation on two benchmark datasets, OV-COCO and OV-LVIS, demonstrates the superiority of our proposed method over existing state-of-the-art approaches in handling the OVD tasks.

==> sections/approach.tex <==
\section{Approach}
% To address open vocabulary object detection, we introduce a prompt enhancement framework to exploit the implicit knowledge of unseen classes in background proposals with the help of PVLMs. Specifically, we propose a prompt enhancement module, which represents the background proposals with multiple open-set class embeddings. An open-set pseudo-labeling strategy is introduced to exploit the unseen classes in implicit objects with the open-set class embeddings. During the inference stage, we devise a probability rectification module to tease apart the competition from open-set classes and accurately estimate the probabilities of novel classes. 
% The overview of our method is illustrated in Fig.~\ref{}.

To tackle the task of Open Vocabulary Object Detection (OVOD), we introduce a prompt enhancement framework to exploit the implicit knowledge of unseen classes in background proposals with the help of PVLMs. Specifically, we propose a prompt enhancement module, which represents the background proposals with multiple open-set class embeddings. An open-set pseudo-labeling strategy is introduced to exploit the unseen classes in implicit objects with the open-set class embeddings. During the inference stage, we devise a probability rectification module to tease apart the competition from open-set classes and accurately estimate the probabilities of novel classes. 
% The overview of our method is illustrated in Fig.~\ref{}.

% To tackle the OVOD task of Open Vocabulary Object Detection (OVOD), we introduce a prompt enhancement framework to exploit the implicit knowledge of unseen classes in background proposals with the help of PVLMs. Specifically, we propose a prompt enhancement module, which represents the background proposals with multiple open-set class embeddings. An open-set pseudo-labeling strategy is introduced to exploit the unseen classes in implicit objects with the open-set class embeddings. During the inference stage, we devise a probability rectification module to tease apart the competition from open-set classes and accurately estimate the probabilities of novel classes. 
The overview of our method is illustrated in Fig.~\ref{}.

\subsection{Preliminaries}
To formalize the problem setting, we define the detection dataset with only annotations of base classes  $\boldsymbol{C}_b$ as $\boldsymbol{D_b}$.
%$\boldsymbol{D_b} = \{(\boldsymbol{I}_i, \boldsymbol{Y}_{i})\}_{i=1}^{N_{b}}$. 
% Here $\boldsymbol{Y}_{i} = \{(c_{j}, \boldsymbol{b}_{j})\}_{j=1}^{N_{i}}$ is a list of $N_{i}$ base class bounding box annotations composed of category labels $c_{j} \in \boldsymbol{C}_b $ and box location $\boldsymbol{b}_{j}$. Here  $N_{b}$ is the number of images in the detection dataset. 
$\boldsymbol{C}_b = \{C_i \}_{i=1}^{n_b}$, where $n_b$ is the number of base classes. 
The detection dataset $\boldsymbol{D_b}$ is used to train an open vocabulary detector with the help of PVLMs.
During the inference stage, this detector is used to detect the objects for both the base classes $\boldsymbol{C}_b$ and novel classes $\boldsymbol{C}_u = \{C_i \}_{i=n_b+1}^{n_b+n_u}$ unseen in $\boldsymbol{D_b}$. $n_u$ denotes the number of novel classes.

In this paper, our framework is built upon the framework of Faster-RCNN\cite{ren2015faster} and traditional distillation-based methods\cite{gu2021open,wang2023object,wu2023aligning}.  In the training stage, for each image, the Faster-RCNN first encodes this image into global image features and generates a set of proposals by a region proposal network. The RoI Head then outputs the proposal embedding for each proposal by performing RoI Align on global image features. In the traditional distillation-based method, the linear classifier is replaced with the cosine classifier with class embeddings output by the CLIP text encoder. Denote the text embedding of class $C_i$ as $t_i$. For a proposal $q$, given the RoI feature $l$ of $q$ , the probability scores $p(i|q) $ of class $C_i(i \in [1, n_b])$ can be estimated by the softmax function,
% \begin{align}
% \label{eq:softmax}
% p(i|q_j)  = \frac{\exp(\alpha \cos(l_j, t_i))}{\sum_{k }^{n_b} \exp(\alpha \cos(l_j, t_k)) + \exp(\alpha \cos(l_j, t_{bg}))}.
% \end{align}
\begin{align}
\label{eq:softmax}
p(i|q)  = \frac{\exp( \cos(l, t_i)/ \tau)}{\sum_{k=1}^{n_b} \exp(\cos(l, t_k)/ \tau) + \exp( \cos(l, t_{bg})/ \tau)}.
\end{align}
Here $t_{bg}$ is the embedding of background class $C_{bg}$ and $\cos$ indicates the cosine similarity function. $\tau$ is the temperature parameter. 
For simplicity, we use function $\mathrm s(\cdot)$ to denote the $\exp(\cos(\cdot)/ \tau)$ .

In the training stage, each proposal $q$ is assigned a category label $y(q)$ based on the labels of ground truth boxes. 
For this proposal $q$, the following cross-entropy loss is applied to optimize the classifier,
\begin{equation}
\label{eq:cross_entropy}
L_{cls}(q) = - \log(p(y(q) |q)).
\end{equation}

%$N_p$ is the number of proposals sampled for this image. 

To better transfer the knowledge of unseen classes from CLIP, existing distillation-based methods propose to align the features of proposals and embeddings output by the image encoder. In this paper. we follow the knowledge distillation module of BARON\cite{wu2023aligning}. 

During the inference stage,  by introducing the text embeddings of novel classes, the detector is capable of detecting the objects of unseen classes $\boldsymbol{C}_u$. For proposal $q$ and its embedding $l$, the probability scores $p(i|q)$ of  class $C_i(i \in [1, n_b + n_u])$ is estimated by,
% \begin{equation}
% p(i|q_j) =  \frac{\exp(\alpha \cos(l_j, t_i))}{\sum_{k = 1}^{n_b+n_u} \exp(\alpha \cos(l_j, t_k)) + \exp(\alpha 
%  \cos(l_j, t_{bg}))}.
% \end{equation}
\begin{equation}
p(i|q) =  \frac{\mathrm s(l, t_i)}{\sum_{k = 1}^{n_b+n_u}\mathrm s(l, t_k) + \mathrm s(l, t_{bg}))}.
\end{equation}
% the backbone first encodes the training image $\boldsymbol{I}_i$ in $\boldsymbol{D_b}$  into features. The features are fed into a region proposal network to output a set of proposals ${b_j}_{j=1}^{n_b}$. $n_b$ is the number. Then the R-CNN head performs RoI Align on to extract proposal embeddings

\subsection{Open-set Prompt enhancement}

As illustrated in Preliminaries, some existing distillation-based methods\cite{gu2021open,wang2023object,wu2023aligning} represent the background class with a single learnable background embedding. However, background proposals consist of a large number of different unseen objects and scenes which exhibit variations in terms of some attributes such as color, size, and appearance. Representing these proposals by a single embedding leads to a loss of information about unseen objects and a conflict with knowledge distillation constraints. To mitigate this problem, DetPro\cite{du2022learning} assumes the distances between embeddings of background proposals and each object class embedding should be equal. Based on this assumption, it proposes to remove the background embedding and devise a soft background loss to force the background to be equally unlike any object class. However, this assumption can be easily violated in the real-world scene where implicit objects often exhibit different similarities to base classes.
An alternative approach to bolster the representation of the background class is to employ multiple diverse open-set class embeddings to represent the unseen classes in background proposals.  
Nevertheless, fully representing the background proposals may need a large number of open-set class embeddings, which may be computationally expensive. Besides, the number of open-set class embeddings is also hard to decide. 
% Nevertheless, the multiple background embeddings may overfit the implicit objects, resulting in a disruption in the estimation of novel class probabilities.
To address these concerns,  we propose an open-set prompt enhancement module, which takes advantage of the aforementioned two mechanisms to represent the background proposals.


We mainly introduce this module under the Vanilla OVD (V-OVD) setting\cite{wang2023object}, where the class names of novel classes are unknown during training and no additional data is provided.
 To better represent the background class, we first construct a set of embeddings to represent the background class, consisting of $n_o$ open-set embeddings $\{t^o_i\}_{i=1}^{n_o}$ and the original background embedding $t_{bg}$.  
Each open-set embedding $t^o_i$ is served to represent an open-set class $C^o_i$, which is unseen in $\boldsymbol{D_b}$. The value of $n_o$ is estimated from the novel object number estimating methods\cite{han2019learning,zheng2022towards} by K-Means clustering, which will be elaborated in the later section. 
 % Each embedding in the implicit object embeddings corresponds to an open set class in background proposals.  So the value of $n_o$ is estimated from the novel object number estimating methods\cite{han2019learning,zheng2022towards}, which will be elaborated in the later section. 
 To further enhance the representability of background embeddings, we extend $\{t^o_i\}_{i=1}^{n_o}$ with a small number $n_a$ of embeddings to be  $\{t^o_i\}_{i=1}^{n_o+n_a}$. Here $n_a$ is a hyper-parameter.  
 % To ensure the  ${t^o_i}_{i=1}^{n_o+n_a}$ represent the objects but not the pure background(e.g. sky), the 
To be consistent with the base class embeddings, we generate all the open-set embeddings $\{t^o_i\}_{i=1}^{n_o+n_a}$ from the text encoder $\mathbb{T}$ of CLIP with the same prompt template. Specifically, we establish a learnable embedding $e_i$ corresponding to the class name of $C^o_i$.  The open-set embedding for $C^o_i$ is estimated by,
\begin{equation}
t^o_i = \mathbb{T}(\mathrm{prompt}(e_i)).
\end{equation}
$\mathrm{prompt}$ indicates the function that concatenates the fixed embeddings of the prompt template and class name $e_i$. 
% All the open-set embeddings $\{t^o_i\}_{i=1}^{n_o+n_a}$ are output by the text encoder of CLIP from learnable embeddings $e_i$ of class name for $C^o_i$,
% \begin{equation}
% t^o_i = T(\mathrm{prompt}(e_i)).
% \end{equation}
% % $e_i$ is the learnable embeddings for the class name and 
% $\mathrm{prompt}$ indicates the function concatenating the fixed embeddings of context and class name $e_i$.  
% Namely, we only learn the class name of each prompt and fix the remaining part. 
The normal background embedding $t_{bg}$ is set as learnable parameters to represent the pure background.


Given the open-set embeddings, we devise a new background loss to enhance the representation of features for background proposals. For a proposal $q$, similar to Eq.~\ref{eq:softmax}, we perform the softmax function on the $\{t_i\}_{i=1}^{n_b} \cup \{t^o_i\}_{i=1}^{n_o+n_a} \cup \{t_{bg}\}$ to obtain the open-set probability scores $p'(i|q)$.  
Here we denote the scores $p'(i|q) (i\in [1, n_b])$ are the probabilities for $\{C_i \}_{i=1}^{n_b}$, the scores $p'(i|q) (i\in [n_b, n_b + n_o+n_a])$ are for $\{C^o_i\}_{i=1}^{n_o+n_a}$ and the last term $p'(n_b + n_o+n_a+1|q)$ is for the background class.

Since a background proposal can be either a proposal with objects in open-set classes or a pure background, the probability of being a background class should be the sum of probabilities of all the open-set classes and the probability of the pure background. Therefore, for a background proposal $q_b$, we apply an open-set background loss,
\begin{align}
p'(bg|q_b) = \sum_{i=n_b}^{n_b+n_o+n_a+1} p'(i|q_b), \nonumber \\ 
L_{bh}(q_b) = - \log( p'(bg|q_b) ).    
\end{align}
This loss enhances the sum of probabilities $p'(bg|q_b)$ of all the open set and background classes and makes the detector softly learn the scores assigned for each open set class and background class.

However, the group of open-set class embeddings and background embeddings may be insufficient to represent all the background proposals with massive different scenes. 
%When a background proposal can not be sufficiently by background embeddings, we consider two scenes: (1) The embedding of the proposal is closer to the embeddings of base classes. In this case, the probabilities for base classes are larger. (2) The proposal dislikes all of the embeddings. 
When a background proposal can not be sufficiently represented by background embeddings, the embedding of $q_b$ is far from any open-set class embedding and the sum of probabilities $p'(bg|q_b)$ should be small.
% the proposals dislike all of the background embeddings. 
In this case, we push the embedding of this proposal equally toward the open-set and background embeddings since the proposals dislike all of the open-set and background embeddings.
%The probability scores should be equally distributed for all background embeddings.
%namely the mean probability of open set classes and background classes is smaller than the mean probability of base classes, 
 When the $p'(bg|q_b) < \gamma$, we incorporate the soft background loss to relax the loss $L_{bh}$ for background proposals.   The final loss $ {bs}$ for the background proposal$q_b$ is formulated as,
% \begin{equation}
% L_{bs}(q_b)=\left\{\begin{matrix}
%  L_{bh}(q_b) &   \textrm{if}\; p'(bg|q_b) < \gamma\textrm{,} \\ 
% - \frac{1}{n_{all}}\sum_{i=n_b}^{n_{all}}\log( p'(i|q_b))   &   \textrm{otherwise.}
% \end{matrix}\right.
% \end{equation}
\begin{equation}
    L_{bs}(q_b) =
    \begin{cases} 
         L_{bh}(q_b),  & \text{if}~p'(bg|q_b) > \gamma, \\
        - \frac{1}{n_{all}}\sum\limits_{i=n_b}^{n_{all}}\log( p'(i|q_b)), &  \text{otherwise}.
    \end{cases}
\end{equation}
Here $n_{all} = n_b+n_o+n_a+1$ represents the number of all embeddings and $\gamma$ is a small threshold.
%and $ \mathrm{soft}(q_j)  = - \frac{1}{n_{all}}\sum_{i=1}^{n_{all}}\log( p'(i|q_j))  $
Compared with soft background loss in DetPro, this loss enhances the reprehensibility by introducing multiple open-set class embeddings to learn from objects of unseen classes and does not need to follow the equally distributed assumption.
It also helps to alleviate the conflict between classification loss and distillation loss.


% Furthermore, we also incorporate an additional background loss with a small loss weight $\lambda_b$ for all the background proposals to encourage the background embeddings $t_{bg}$ to learn the class-agnostic knowledge from background proposals. For each background proposal $q_b$, we perform softmax on $\{t_i\}_{i=1}^{n_b} \cup \{t_{bg}\}$ to obtain close-set probability scores $p(i|q_b)$  as in Eq.~\ref{eq:softmax}. We denote the $p(bg|q) = 1 - \sum_{k=1}^{n_b} p(k|q)$ as the probability for background class.
% The loss is formulated as the following function, 
% % Furthermore, we also incorporate an additional background loss with a small loss weight $\lambda_b$ for all the background proposals to encourage the background embeddings $t_{bg}$ to learn the class-agnostic knowledge from background proposals.  For the background proposal $q_b$,  we calculate the cross-entropy loss with base class embeddings and the background embeddings $t_{bg}$,
% \begin{equation}
% L_{cls}^b(q_b) = - \lambda_b \log(p(bg|q_b)).
% \end{equation}
% % Note that the open-set class embeddings are not involved in the estimation of this loss.

% For a foreground proposal $q_f$, we apply the cross-entropy loss as,
% \begin{equation}
% L_{cls}^f(q_f) =-  \log(p'(y(q_f)|q_f)).
% \end{equation}
% Here $y(q_f)$ is the assigned label of $q_f$.







\noindent\textbf{Estimation of $n_o$} We first generate the proposals for all the training images from the class-agnostic RPN trained by base detection dataset$\boldsymbol{D_b}$ as in VL-PLM\cite{zhao2022exploiting}. 
These proposals are filtered by RPN scores with a threshold of $\theta_{r}$ and per-class non-Maximum Suppression(NMS).
Instead of using RoI features, we generate the features from the image encoder of CLIP for these proposals to obtain a set of embedding features ${l}^o$.  Finally, we use the novel object number estimating methods\cite{han2019learning,zheng2022towards} to choose the best $n_o$ by applying the K-means clustering\cite{duda1973pattern} on the generated features of all the proposals.

\subsection{Open-set Pseudo labeling}
To better discover and exploit unseen objects, we propose an online pseudo-labeling strategy to mine the implicit objects for open classes in background proposals. At the beginning of training, given the $n_o$, we first perform K-means clustering on the embedding set ${l}^o$, obtaining the cluster centers $\{m_i\}_{i=1}^{n_o}$.  The cluster centers $\{m_i\}_{i=1}^{n_o}$  can serve as centers of open-set classes to generate the pseudo labels online from background proposals in each batch. 
During the training process, encouraged by VL-PLM\cite{zhao2022exploiting}, the background proposals in each batch are filtered by RPN scores with the threshold of $\theta_r$ and the proposals with overlaps with ground truth boxes are filtered. Then, we use the CLIP to generate pseudo labels to prevent the detector from overfitting with the open-set class.
For a background proposal $q_b$, the embedding $l^c_b$ is output by the image encoder of CLIP from the region of $q_b$ as in \cite{wu2023aligning}. The probability score of $q_b$ belonging to the  open set class $C^o_i(i \in [1, n_o])$ is calculated as, 
\begin{equation}
p^o(i|q_b) =   \frac{\mathrm s(l^c_b, m_i)}{\sum_{k = 1}^{n_b} \mathrm s(l'_b, m_i)}.
\end{equation}
% \begin{equation}
% p^o(i|q_j) =   \frac{\exp(\alpha \cos(l'_j, m_i))}{\sum_{k = 1}^{n_b} \exp(\alpha \cos(l'_j, m_i)))}.
% \end{equation}
The open class with the maximum probability is set as the pseudo label $y^o(q_b) \in [n_b, n_b+n_o]$  of $q_b$. To eliminate the unconfident pseudo labels,  the proposals are filtered by the scores of pseudo labels by a threshold $\theta_o$. Following VL-PLM\cite{zhao2022exploiting}, we apply per-class NMS and use the RoI head to refine the box prediction to generate final pseudo labels. We use the final pseudo labels to assign the open-set labels for all the background proposals $Q^{b}$ in a batch. Denote the set of positive background proposals assigned with open-set labels as $Q^{bf}$ and the set of remaining background proposals as $Q^{bb}$.
The final loss for the pseudo-labeling strategy is defined as the following equation,
\begin{align}
L_{ps} =  \frac{1}{|Q^{bf}|} \sum_{q \in Q^{bf}} -\log(p'(y^o(q)|q)) \nonumber \\
+ \lambda_{bg} \frac{1}{|Q^{bb}|}  \sum_{q \in Q^{bb}}-\log(\sum_{i=n_b+n_o}^{n_{all}}p'(i|q)).
\end{align}
$\lambda_{bg}$ is a small weight for background. This loss encourages the open set embeddings to fit the open set classes in the background proposals, especially for the majority classes which suffer more from loss of knowledge.
Besides, with this pseudo-labeling strategy, the detector can also exploit the knowledge from the implicit objects.

\noindent \textbf{Training Objective.} The final objective for model optimization is a combination of the proposed training losses stated above,
\begin{align}
L = \frac{1}{|Q^{b}|}\sum_{q \in Q^{b}} (L_{cls}^b(q) + L_{bs}(q)) + \nonumber \\
 L_{ps}  + \frac{1}{|Q^{f}|}\sum_{q \in Q^{f}} L_{cls}^f(q).
\end{align}
$Q^{f}$ and $Q^{b}$ are the set of all the foreground proposals and background proposals in a batch respectively.
% $N_p$ is the number of proposals sampled for this image. 
%$L_{cls}^f$ is the cross-entropy loss for foreground proposals as in Eq.~\ref{eq:cross_entropy}.


\subsection{Probability rectification}
The integration of the prompt enhancement and pseudo-labeling methodologies serves to augment the capacity of open-set embeddings in capturing the characteristics of previously unseen classes.
 Nonetheless, a challenge arises in situations where unseen classes $\{C^o_i\}_{i=1}^{n_o+n_a}$  exhibits overlap with the novel classes $\boldsymbol{C}_u$, which are the classes detector aims to detect. In such instances, a conflict emerges as the embeddings for open-set classes vie with those for the novel classes during the inference stage. This competition impedes the accurate estimation of scores for the novel classes, introducing ambiguity in the recognition process. To address this issue, we introduce a probability rectification mechanism to refine the inference stage.

During the inference stage, the probability score of a proposal $q$  belonging to class $C_i(i \in [1, n_b + n_u])$ is estimated by,
\begin{equation}
p(i|q) =  \frac{\mathrm s(l, t_i)}{\sum\limits_{k = 1}^{n_b+n_u}\mathrm s(l, t_k) + \sum\limits_{k = 1}^{n_o+n_a}\mathrm s(l, t^o_k)  + \mathrm s(l, t_{bg})}.
\end{equation}
$l$ is the ROI feature of $q$.
Since the $\{C^o_i\}_{i=1}^{n_o+n_a}$ may overlap with $\boldsymbol{C}_u$, the part of exponential scores of novel classes are duplicated estimated in the denominator of above softmax function.
Thus, $p(i|q)$ is biased from the real probability $\mathrm P(q \in C_i|q)$.  To address this problem, the impact of open-set classes should be eliminated from the scores of the novel classes. For simplicity, we denote $\mathrm P(q \in C|q)$ as $\mathrm P(C|q)$ for arbitrary class $C$.

% For each open set class $C^o_k$, we aim to transfer the $C^o_k$ to $C^n_k$, which does not overlap with $\boldsymbol{C}_u$. 
% We expect there is $P(C^n_k|q) = P(q \in C^o_k, q \notin  {C}_u|q)$.
% To rectify the probability in the softmax function, we propose to estimate the exponential scores $\mathrm s(l, C^n_k)$ for $C^n_k$. Since the softmax function estimates the probability for each class by dividing each exponential score by the sum of exponential scores, we consider the exponential scores to be proportional to the real probabilities for each proposal. 
% 对于任意一个潜在类别 $C^o_k$, 我们需要去移除其中与novel类$\boldsymbol{C}_u$相关的部分。我们将移除后$C^o_k$剩下的的部分称为类别$C^n_k$。其中，p属于$C^n_k$的一个样本的概率为$P(C^n_k|q) = P(q \in C^o_k, q \notin  {C}_u|q)$。 因为我们最终是要估计一个正确的softmax分+母，所以我们只需要考虑计算$C^n_k$对应的指数分数。对于softmax function中的每一类，它的概率分数










Based on this, the $\mathrm s(l, C^n_k)$ is estimated by,
% can be $\mathrm s(l_j, C^n_k)$.
% we assume $\mathrm s(l_j, t_j) = \beta P( C^o_k|q_j)$ and $\mathrm s(l_j, C^n_k) = \beta P( C^o_k|q_j)$.
% With the softmax function, $\mathrm s(l_j, t_j) / \sum_{t} \mathrm s(l_j, t) $ can represent the $P(q_j \in C^o_k|q_j)$.
% With the softmax function, we consider the $\mathrm s(l_j, t_j) = \beta P(q_j \in C^o_k|q_j)$ and $\mathrm s(l_j, t_j) = \beta P(q_j \in C^o_k|q_j)$.
% Thus, we eliminate the part of  $\mathrm P( C^o_k, q_j \in \boldsymbol{C}_u|q_j)$ in $\mathrm s(t^o_k, l_j)$  and preserve the part of probability $\mathrm P(C^o_k, q_j \notin \boldsymbol{C}_u|q_j)$ to get the scores $\mathrm s(l_j,C^n_k)$ for  $C^n_k$,
\begin{equation}
\label{eq:distinct}
\mathrm s(l, C^n_k) = s(l, t^o_k)  (1 - \frac{\sum_{i=n_b}^{n_b+n_u}\mathrm P(C_i, C^o_k|q)}{\mathrm P( C^o_k|q)}).
\end{equation}


To estimate the overlap part $\mathrm P(C^o_k,  C_i|q)$, we have the following equation,
\begin{equation}
\mathrm P( C^o_k,  C_i|q) =  \mathrm P( C^o_k|q)  \mathrm P( C_i|q, C^o_k). 
\end{equation}
The Eq.~\ref{eq:distinct} can be transferred to,
\begin{equation}
\label{eq:distinct_v2}
\mathrm s(l, C^n_k)=  s(l, t^o_k) ( 1 - \sum_{i=n_b}^{n_b+n_u}P( C_i|q, C^o_k)) .
\end{equation}
However, $\mathrm P( C_i|q, C^o_k)$ is hard to estimate. So we assume the $\mathrm P( C_i|q, C^o_k)$ is sample-agnostic, obtaining $P( C_i|q, C^o_k) = P( C_i| C^o_k)$. 
% #如前面讨论的一样，分类器通过计算proposal的RoIfeature和一个类别的class embedding之间的相似性并通过softmax来计算这个proposal属于这个类别对应的概率。那么同样的，我们认为通过对每个类$C^o_k$和$C_i$d做同样的操作可以一定程度反映属于$C^o_k$的样本属于类别$C_i$的概率。
dince the embeddings space is used as a metric space to calculate the probability, $P( C_i| C^o_k)$ can be also estimated based on the similarity of embeddings,
\begin{equation}
\label{eq:inclass}
P( C_i|q, C^o_k) = P( C_i| C^o_k) = \frac{\mathrm s(t^o_k, t^i)}{\sum\limits_{t \in {t}^{all}, t \neq t^o_k }\mathrm s(t^o_k, t)}.
\end{equation}
${t}^{all}$ denotes all the embeddings $\{\{t_i\}_{i=1}^{n_b+n_u} \cup \{t^o_i\}_{i=1}^{n_o+n_a} \cup \{t_{bg}\}\}$.
According to Eq.~\ref{eq:inclass} and Eq.~\ref{eq:distinct_v2}, the $\mathrm P(C_i|q_j)$ can be obtained by,
\begin{equation}
P( C_i| q) =   \frac{\mathrm s(l, t_i)}{\sum\limits_{k = 1}^{n_b+n_u}\mathrm s(l, t_k) + \sum\limits_{k = 1}^{n_o+n_a}\mathrm s(l, C^n_k)  + \mathrm s(l, t_{bg})}.
\end{equation}
% The probability rectification helps to estimate the probabilities for novel classes more accurately when the open set classes overlap with novel classes.
The probability rectification facilitates a more accurate estimation of probabilities of novel classes, mitigating potential ambiguities that may arise when the open-set and novel class sets intersect.

% \subsection{Prompt enhancement under Generalized OVD  }

==> sections/experiments.tex <==
\section{Experiments}
\subsection{Datasets} 
Our method is evaluated on the two benchmark object detection datasets,  MS-COCO \cite{lin2014microsoft} and LVIS \cite{gupta2019lvis} in the traditional open vocabulary settings \cite{gu2021open,wang2023object,wu2023aligning}.
We indicate the open-vocabulary setting based on MS-COCO and LVIS datasets as OV-COCO and OV-LVIS, respectively.
For the OV-COCO task, following \cite{wang2023object,wu2023aligning},  we split 48 categories into base classes and 17  categories into novel classes.
% To validate the effectiveness of our method, we report the performance of detectors 
The main metric to validate the performance of detectors is the mean average precision at IoU threshold 0.5 (note as $\textrm{AP}_{50}$). The $\textrm{AP}_{50}$ on base and novel are denote as $\textrm{AP}^n_{50}$  and $\textrm{AP}^b_{50}$, respectively.  
For the LVIS task, following \cite{wang2023object,wu2023aligning},  the 337 rare categories are selected as novel categories and the remaining common and frequent categories are into base categories (866 categories).  The performance of detectors is validated in the mean average precision averaged on IoUs from 0.5 to 0.95, noted as $\textrm{AP}$. We report the $\textrm{AP}$ of rare categories $\textrm{AP}_r$, common categories $\textrm{AP}_c$,  frequent categories $\textrm{AP}_f$ and all classes. 
The results for instance segmentation are also reported in the LVIS dataset. 
$\textrm{AP}^n_{50}$  and $\textrm{AP}_r$ are the main metrics to evaluate the performance of open vocabulary detectors on OV-COCO and OV-LVIS, respectively.
% Following previous methods\cite{radford2021learning,wu2023aligning}, we also report the performance of the detector trained on OV-LVIS on three other datasets, namely the  Pascal VOC 2007\cite{everingham2010pascal}, MS-COCO\cite{lin2014microsoft}  and Objects365\cite{shao2019objects365}. 


\subsection{Implemental details}
We conduct the experiments on the framework of BARON\cite{wu2023aligning}. Following previous work\cite{radford2021learning,wu2023aligning}, we select Faster RCNN \cite{ren2015faster} with ResNet50-FPN \cite{lin2017feature} as our base detector. The weights of the backbone network are initialized by SOCO\cite{wei2021aligning}.  We train the network with $2\times$ schedule(180000 iterations) with a batch size of 32(16 for detection and 16 for distillation) for OV-LVIS. 
Stochastic gradient descent (SGD)~\cite{ruder2016overview} is selected as our optimizer with the momentum set to 0.9 and the weight decay set to $ 2.5\times 10^{-5}$. Following Baron\cite{wu2023aligning}, we adopt the ViT-B/32
CLIP\cite{dosovitskiy2020image} as the PVLM. The fixed context of the prompt is set to the simple template in ViLD\cite{gu2021open}.
 Following VL-PLM\cite{zhao2022exploiting}, the thresholds $\theta_r$ and $\theta$ are both set to 0.95. $\gamma = $ and $\lambda_{bg} = 0.05$.


\subsection{Comparisons on the OV-COCO task}
We conduct the experiments on  OV-COCO tasks to compare our method against  existing OV-COCO methods, including Detic\cite{zhou2022detecting}, Object-centric-OVD\cite{bangalath2022bridging}, OV-DETR\cite{zang2022open}, RegionCLIP\cite{zhong2022regionclip}, ViLD\cite{gu2021open},
OADP\cite{wang2023object} and BARON\cite{wu2023aligning}. The results are shown in Tab.~\ref{tab:OV-COCO}. Following OADP, we categorize these methods into four OVD benchmark settings: Vanilla OVD (V-OVD), Caption-based OVD (C-OVD), Generalized OVD (G-OVD), and Weakly Supervised OVD (WSOVD).
Our method mainly focuses on the V-OVD setting. For completeness, we also report the performance of methods in other settings. For a fair comparison, we reimplement the BAROM as BARON* with a smaller batch size of $16$, which is beneficial to alleviate the overfitting on the base classes.

The results in Tab.~\ref{tab:OV-COCO} show our method outperforms all the existing OVD methods by a clear margin in the V-OVD setting. Concretely, our method effectively boosts the performance of BARON* by 2.0\% on $\textrm{AP}^n_{50}$ and 0.5\% on $\textrm{AP}^b_{50}$.  It shows our prompt enhancement can better represent the background proposals, which is beneficial to the learning of representations of both base classes and novel classes. Furthermore, the performance of our method also surpasses most of the OVD methods on other OVD in other benchmarks even without any prior knowledge. It demonstrates the generality and superiority of our method.

\input{tables/OV-COCO} 

\subsection{Comparisons on the OV-LVIS task}
We also compare the performance of our method on OV-LVIS tasks with several existing OV-COCO methods, including ViLD\cite{gu2021open}, DetPro\cite{du2022learning} and BARON\cite{wu2023aligning}. Compared to OV-COCO, OV-LVIS is more challenging due to the much larger number of classes and fewer implicit instances for novel classes in the detection dataset. Following Baron, we report the performance with and without the learnable prompts in DetPro.
The results in Tab.~\ref{tab:OV-LVIS} showcase the superior performance of our method. For the object detection task, our method achieves substantial improvements of  2.1\%  without learnable prompts and 0.9\%   with learnable prompts for BARON on $\textrm{AP}_{r}$. For instance segmentation task, our method consistently improves the performance of BARON by 2.9\% on $\textrm{AP}_{r}$.
These comparisons demonstrate that our method can be applied to more challenging object detection tasks with a large number of classes.
\input{tables/OV-LVIS}

% \input{tables/OV-transfer}

\subsection{Ablation study}
\textbf{Effectiveness of our core components.}
To understand the effect of each component in our method, i.e. open-set prompt enhancement(OSPE), open-set pseudo labeling(OSPL) and probability rectification(PR),
we conduct the ablation study by incrementally incorporating these modules. The results are presented in Tab.~\ref{tab:ablation_components}.  It can be observed that only employing OSPE significantly improves the baseline's performance on the base classes while resulting in a decline in the performance of the novel classes.  his observation underscores that the exclusive application of OSPE is susceptible to competition between underlying classes and novel classes. When incorporating the PR along with OSPE, the performance of novel classes improves by 2.5\%, demonstrating the effectiveness of PR. The further application of OSPL brings 1.0\% mAP50 performance gain on novel classes, which validates the effectiveness of OSPL on better discovering the underlying classes.

\input{tables/Ablation_components}

\noindent \textbf{Analysis of background interpretation methods.}
To validate the effectiveness of the proposed OSPE, we ablate different ways for background interpretation in Tab.~\ref{tab:ablation_bg}. We denote the 'Single embedding' as using only a single background embedding $t_{bg}$ as in previous methods\cite{gu2021open,wu2023aligning}. 'Soft background loss' indicates the soft background loss in DetPro\cite{du2022learning}. $L_{bh}$ and $L_{bs}$ denotes we replace the loss for background proposals $L_{cls}^{b} + L_{bs}$ with only $L_{bh}$ and $L_{bs}$, respectively.
The results clearly show that our background interpretation method is superior to other background interpretation methods. Concretely,  our method outperforms 
soft background loss by a clear margin. It means our method better represents when maintaining the class-wise relations. Besides, the comparison with only employing $L_{bh}$ and $L_{bh}$ demonstrates the importance of each loss in our background losses.


We also visualize the features and base class similarities of novel class proposals with t-SNE in Fig.~\ref{} to further illustrate the effectiveness of our background interpretation. For a novel proposal $x$ with visual embedding $\textit{\textbf{w}}{(x)}$ from RoI head, we define the base class similarity for class $c \in \mathcal{C}_b$ by $\textit{\textbf{w}}{(x)}$ to reflect the class relations with base classes. The normalized base score used for visualization for each proposal is a vector that concentrates the normalized base class score for each class $c \in \mathcal{C}_b$.
Compared to the background interpretation with a single embedding in the baseline, our method learns more discriminative features for novel class proposals.  The comparison between Fig~\ref{fig:t-SNE-c} and Fig~\ref{fig:t-SNE-d} shows our method exhibits a more diverse distribution on normalized base scores and effectively maintains the class relation between the underlying classes and base classes.

% We also visualize the features and normalized base class scores of novel class proposals with t-SNE in Fig.~\ref{} to further illustrate the effectiveness of our background interpretation. For a novel proposal $x$ with visual embedding $\textit{\textbf{w}}{(x)}$ from RoI head, we define the normalized base class score for class $c \in \mathcal{C}_b$ by $p(c|x; \mathcal{C}_b)$ to reflect the class relations with base classes. The normalized base score used for visualization for each proposal is a vector that concentrates the normalized base class score for each class $c \in \mathcal{C}_b$.
% Compared to the background interpretation with a single embedding in the baseline, our method learns more discriminative features for novel class proposals. 
% The comparison between Fig~\ref{fig:t-SNE-c} and Fig~\ref{fig:t-SNE-d} shows our method exhibits a more diverse distribution on normalized base scores and effectively maintains the class relation between the underlying classes and base classes.
%The comparison between Fig~\ref{fig:t-SNE-c} and Fig~\ref{fig:t-SNE-d} demonstrates our method effectively maintains the class relation between the underlying classes and base classes.
\input{figures/t-SNE}

\input{tables/Ablation_background}

\noindent \textbf{Ablation of probability rectification.}
To further validate the performance of probability rectification, we also perform comparisons with some variants of probability rectification. As shown in Tab.~\ref{tab:ablation_pr}, equally teasing apart all the underlying class embeddings(Note as w/o $t^o_k$) for softmax function obtain a decline of -0.1\%  on $\textrm{AP}^n_{50}$ and -0.9\% on $\textrm{AP}^n_{50}$ compared to the baseline method. 
This method eliminates not only the joint part but also the disjoint part with novel classes in the scores of underlying classes.  
In contrast, our probability rectification enhances the performance by 2.2\% by maintaining the scores of underlying classes disjoint with novel classes.
\input{tables/Ablation_pr}

% \noindent  \textbf{The performance under different $n_a$.}


==> sections/introduction.tex <==
\section{Introduction}
% Recently, Pretrained Vision-and-Language Models (PVLMs) have witnessed marvelous success for their great generalizability to adapt to downstream tasks. With the help of  PVLMs,  Open-vocabulary object detection (OVD)  become a new rising topic. It aims to transfer knowledge from PVLMs to detection tasks so that the detector can detect unseen objects beyond the annotated detection dataset in a zero-shot manner. With the capability of detecting new classes without annotations, OVD is of great significance in real-world scenes.

% In recent times, Pretrained Vision-and-Language Models (PVLMs)\cite{radford2021learning,jia2021scaling} have demonstrated remarkable success due to their exceptional generalizability when applied to downstream tasks. With the capability of PVLMs, Open-vocabulary object detection (OVD) has emerged as a burgeoning area of study. The core objective of OVD is to facilitate the transfer of knowledge from PVLMs to object detection tasks, enabling detectors to identify previously unseen objects without the need for specific annotations.  The capacity to detect novel classes in the absence of explicit annotations renders OVD particularly consequential for real-world scenarios and applications.
Object detection has witnessed significant success in research, such as~\cite{ren2015faster, lin2017feature, shao2019objects365, zheng2022towards}, however, solely detecting and classifying objects within known categories (base classes) during inference significantly diminishes its generalization capacity in real-world applications. Open Vocabulary Object Detection (OVOD) emerges as a prospective means to overcome this restriction, endowed with the capability to detect unseen categories (novel classes), without the explicit need for annotations.
Leveraging pre-trained Vision and Language Models (PVLMs), exemplified by CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling}, recent advances in OVOD, e.g.~\cite{gu2021open, du2022learning, wu2023aligning}, employ knowledge distillation to transfer insightful knowledge of PVLMs to the task of object detection, generalizing its powerful capabilities to detect more unknown object categories. 
 % The target of the OVD is to enable the detector to detect both base and novel categories by transferring knowledge from PVLMs, where the base categories are only annotated in the training set. 

% One of the mainstream methods within OVD is the distillation-based method. These methods introduce knowledge distillation by aligning the features of proposals from the detectors with the features from the image encoder of CLIP\cite{radford2021learning}. By mimicking the feature space of detectors to the feature space of PVLMs, detectors are capable of detecting unseen objects not learned before.

Leveraging PVLMs, recent advances in OVOD, e.g.~\cite{gu2021open, du2022learning, wu2023aligning}, employ knowledge distillation to align the features of proposals generated by the detector with those extracted by the image encoder of PVLMs. 
%Once the coherence between the feature spaces of the detector and PVLMs is forced, implicitly projecting the visual features of the detector to the textual embedding space of PVLMs.
In this way, the object detector implicitly learns the knowledge of rich and unseen categories from large-scale vision-concept pairs of PVLMs.
However, these methods mainly focus on exploiting a more effective knowledge distillation mechanism but lack a careful design to interpret the background class, leading to a loss of intra-background knowledge. 
% The research effort toward designing an effective background interpretation and background exploration scheme remains severely under-explored.
%but ignore the design of effective background interpretation scheme. 
Concretely, traditional distillation-based approaches\cite{gu2021open,wu2023aligning}  tend to interpret background class using a single learnable embedding, which inadequately captures the extensive diversity in background proposals.
Consequently, it results in the loss of critical intra-background information.  In addressing this limitation, some researchers apply multiple binary classifiers\cite{bangalath2022bridging} or devise a soft background loss\cite{du2022learning} to equally push the background proposals away from foreground embeddings without learning the background embedding. However, they assume the background proposals to be equally unlike the foreground classes, which ignores the relations between the foreground class and the underlying classes as illustrated in Fig.~\ref{fig:teaser}. 
% As illustrated in Fig.~\ref{fig:teaser}, the embedding of an unseen object of TV from CLIP is naturally closer to the class embeddings of the laptop.
% The indiscriminate pushing of embeddings equally away from all class embeddings can disrupt the learning of nuanced relationships between classes. 
Furthermore, existing methods encounter challenges in fully transferring the knowledge of novel classes to the detector through knowledge distillation. In contrast, the detector readily acquires knowledge of base classes owing to a substantial volume of fully-supervised data, leading to an imbalance that contributes to the overfitting of the detector on the base classes
%since existing knowledge distillation methods hard to fully transfer the knowledge from PVLMs. 
%Compared to the base class with  fully supervised annotations, the knowledge 
% Besides, the OVOD detectors tend to overfit the base classes with sufficient annotations for detection.
%As illustrated in Fig.~\ref{}, the embedding of an unseen object of TV should be naturally closer to the class embedding of the laptop since the TV is more similar to the laptop in appearance.
%The indiscriminate pushing of embeddings equally away from all class embeddings can disrupt the learning of nuanced relationships between classes.
% Otherwise, some methods\cite{} apply multiple binary classifiers for the classification branch. They also push away from background proposals equally, neglecting the class relations between seen and unseen classes.


% However, two primary challenges impede the effective representation of features in distillation-based methods: (1) The insufficient representations of background proposals by existing prompting methods\cite{han2019learning,ren2023prompt}. 
% % Traditional methods\cite{gu2021open,wu2023aligning} represent the background classes by a single learnable embedding, which is insufficient to represent massive diverse proposals and leads to a loss of intra-background information. 
% Traditional approaches\cite{gu2021open,wu2023aligning}  tend to represent background classes using a single learnable embedding, which inadequately captures the extensive diversity in background proposals.
% % This fails to account for variations in background attributes, such as color, size, and appearance. 
% Consequently, it results in the loss of critical intra-background information. 
% In addressing this limitation, DetPro\cite{han2019learning} devise a soft background loss to equally push the background proposals away from foreground embeddings. However, they assume the background proposals to equally dislike the foreground classes, which ignores the relations between the foreground class and the implicit objects. 
% As illustrated in Fig.~\ref{}, the embedding of an unseen object of TV should be naturally closer to the class embedding of the laptop since the TV is more similar to the laptop in appearance. The indiscriminate pushing of embeddings equally away from all class embeddings can disrupt the learning of nuanced relationships between classes.
% Otherwise, some methods\cite{} apply multiple binary classifiers for the classification branch. They also push away from background proposals equally, neglecting the class relations between seen and unseen classes.  
% %These insufficient representations not only lead to a loss of but also cause a conflict with knowledge distillation.
% (2)  Overfitting on the base classes with sufficient annotations for detection.
% PVLMs are primarily pre-trained using contrastive learning on image captions and images and thereby unaware of precise object localization information, a crucial aspect of successful object detection.  Therefore, the detectors still lack sufficient detection knowledge of unseen objects and overfit the base classes with annotations for detection. 
%The gap between the knowledge from PVLMs and the knowledge required for the detection task.
% The under-explorations of implicit objects in the detection dataset. 
% A significant factor contributing to this issue is the disparity between the knowledge derived from PVLMs and the knowledge essential for object detection.  PVLMs are primarily pre-trained using contrastive learning on image captions and images and thereby unaware of precise object localization information, a crucial aspect of successful object detection.
% The PVLMs are pre-trained by contrastive learning to match the image captions and the corresponding images. So the features from PVLMs are unaware of the accurate positions of objects, which are essential for objedetection.
% PVLMs are primarily pre-trained using contrastive learning to align image captions with their corresponding images. Consequently, the features extracted from PVLMs inherently lack precise object localization information, a crucial aspect of successful object detection tasks. 
% Thus, in the training process on the detection dataset, the detectors still lack sufficient detection knowledge of unseen objects and overfit the base classes with annotations for detection. 

% We propose to tackle the two obstacles from a new perspective:
% Pseudo-labeling is a simple but effective way to alleviate the two challenges.
To address these problems, some approaches\cite{zhao2022exploiting,bangalath2022bridging} propose to mine the implicit objects for novel classes from background proposals to perform pseudo-labeling on the detection dataset. By introducing class embeddings for novel classes, these methods enhance the interpretation of objects from novel classes present in the background. However, the knowledge beyond the novel classes remains largely unexplored. Furthermore, this type of method relies on additional prior knowledge such as the name of novel classes or the additional weakly supervised data, which limits the application of these methods.

We materialize these motivations and propose to address the two challenges from a new perspective: Since the background proposals involve a large number of objects of underlying classes, learning to discover and represent the underlying classes is beneficial for interpreting the background class.  By further classifying the background proposals into different classes, the detector is able to capture the variability between different underlying classes and learn the more discriminative representations for background proposals.  Additionally, discovering the objects of these underlying classes enables pseudo-labeling without any prior knowledge, thereby contributing to the prevention of model overfitting.
% Besides, the pseudo-labeling methods can be performed without  to alleviate the overfitting of detector.
%is beneficial for the detector to represent the background class and exploit the knowledge from implicit objects. 
% By aligning the embeddings of objects to their corresponding open-set prompt embeddings, the class relations among both base classes and open-set classes are better preserved. 
% Besides, prompting the open set classes enables the pseudo labeling on unseen classes.  It helps to better transfer the knowledge from PVLMs for detection and alleviates the overfit of detectors on base classes.
% Besides, exploiting the knowledge from the unseen classes helps to alleviate the overfitting to base classes without the need for any prior knowledge.
% The background class can be better represented by learning to prompt the open set classes which are unseen in the annotations of the detection dataset.
Motivated by these, we propose a new prompt-enhancement framework, involving an open-set prompt enhancement module, an open-set pseudo-labeling module and a probability rectification module. The open-set prompt enhancement module learns to prompt the open-set classes and generate a set of open-class embeddings to extend the embeddings for the background. We also incorporate the soft background loss to relax the loss for the objects beyond the open-set classes.
% extends the background embedding with a set of open-class embeddings output by the text encoder from a group of learnable prompts for open-set classes. 
% For the proposals hard to be represented by these embeddings, we also introduce the soft background loss to mitigate the information loss. 
To better discover and exploit the unseen classes, the open-set pseudo-labeling module clusters the feature of background proposals to discover the unseen classes and generates pseudo labels for each open-set class with CLIP. During the inference stage, the probability rectification module is further introduced to eliminate the competition between open-set classes and desired novel classes. Our contributions can be summarized as follows:
\begin{itemize}
    \item We start from a new perspective of discovering and prompting the unseen classes in the background and design a prompt enhancement framework for implicit objects.
    \item We introduce a prompt enhancement module along with the probability rectification module to represent the open-set classes when maintaining the intra-background attributes and class-wise relations.
    \item An open-set pseudo-labeling strategy is designed to better represent the unseen classes, which helps to alleviate overfitting.
    \item  Extensive experiments on two benchmark OVD tasks OV-COCO and OV-LVIS  show that our method can boost the performance of existing distillation-based methods, demonstrating the superiority of our method.
\end{itemize}


==> sections/related.tex <==
\section{Related works}
% \subsection{Open-vocabulary object detection} 
With the advent of Pretrained Vision-and Language Models (PVLMs), Open vocabulary object detection (OVOD) has seen notable progress in recent years  \cite{du2022learning,yao2023detclipv2,,zang2022open,wu2023cora} . 
It aims to train a detector that can detect both the objects annotated in the detection dataset and the objects seen and unseen in the detection dataset by transferring knowledge from PVLMs.
% It aims to train a detector that can detect both the objects annotated in the detection dataset and the objects unseen in the detection dataset by transferring knowledge from PVLMs. 

% \noindent
\textbf{OVOD based on Fine-tuning.}
OVR-CNN \cite{zareian2021open} first proposes the problem and extends the object detection capabilities with the image-caption dataset. Notably, recent attempts push forward this direction mainly by fine-tuning the PVLMs to adapt the detection task or distilling knowledge from CLIP\cite{radford2021learning} to the detector. RegionCLIP\cite{zhong2022regionclip} fine-tunes the CLIP model by establishing the region-text pair.  GLIP\cite{li2022grounded} unifies the detection and grounding tasks. It generates massive image-text pairs by self-training strategy for pretraining. However, this type of method needs to re-train the large vision and language Models, which is time-consuming and computationally expensive.

% \noindent
\textbf{OVOD based on distillation.}
In contrast, the knowledge-distillation-based methods mainly follow the source-free manner. ViLD\cite{gu2021open} first employs knowledge distillation by aligning the features from detectors and embeddings output by CLIP. BARON\cite{wu2023aligning} generates bags of regions by randomly masking the region in grids for distillation to learn the co-existence of visual concepts in a scene. Although these methods transfer the knowledge of novel classes from PVLMs to some extent, the detectors are still biased toward base classes due to the gap between vision-language matching and detection tasks. To address it, some researchers focus on applying pseudo labeling\cite{zhao2022exploiting} with prior knowledge about novel class names or introducing additional weak-supervised annotations for detection dataset\cite{zhou2022detecting,bangalath2022bridging}. The utilization of additional knowledge limits the application of these methods in real-world scenes. 

Our method can effectively exploit the implicit knowledge of unseen classes in the detection dataset without any prior knowledge about novel classes, which is of more generality.

% One of the early directions in this field was zero-shot learning, which focused on extending the object detection capabilities beyond predefined categories using semantic embeddings of objects. Additionally, , such as CLIP, has ushered in a new era. These models leverage text and image embeddings to perform open-vocabulary object detection, serving as a foundation for various approaches. Notably, many methods have arisen that capitalize on CLIP's capabilities for translating textual queries into image embeddings and enhancing detection accuracy. Some approaches employ graph-based models, which create a semantic space connecting textual and visual information, while others investigate scalable vocabularies and large-scale pretraining to expand the range of recognizable objects. Multimodal fusion techniques have also gained prominence by leveraging both textual and visual information for improved object localization. Overall, these works reflect the dynamic evolution of open-vocabulary object detection, paving the way for enhanced capabilities in the recognition of objects based on user-defined textual descriptions

% \noindent \textbf{Open-set object detection and novel object discovery}

% \subsection{Prompt tuning}
% \noindent
\textbf{Prompt tuning related to OVOD.}
Prompt tuning first derives from natural language processing. With the development of the VPLMs, prompt tuning\cite{,khattak2023maple} has been introduced to enhance the efficacy of VPLMs for specific downstream tasks. CoOp\cite{zhou2022learning} first proposes the learnable contexts for prompting into 2D vision-language classification. CoCoOp\cite{zhou2022conditional}  extends CoOp by further generating an input-conditional token for each image. Besides, some visual prompting methods\cite{jia2022visual,bahng2022visual,guo2023viewrefer,chen2023visual} propose to add the prompt for the image encoder.
In open vocabulary object detection, DetPro\cite{radford2021learning} first applies prompt engineering and designs a soft background loss to force the background proposals to dislike the base class embeddings equally. \cite{ren2023prompt} propose to pre-train prompts with a massive class set to generate universal prompts with better generality. 
Different from DetPro, our method does not follow the equally distributed assumption and can better learn a representation for background class by prompting the open-set classes.
%further exploit the knowledge in background proposals.
% With the development of the large language model

==> tables/Ablation_parameters.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l|ccc}
% \hline
\toprule
$n_a$  &   $\textrm{AP}^n_{50}$ & $\textrm{AP}^b_{50}$ & $\textrm{AP}_{50}$   \\ 
% \hline
\midrule
$0$ &  37.5 & 58.5  & 53.0  \\ 
$10$ & 37.8 & 58.7 & 53.2\\ 
$20$ & 37.7  & 58.7    & 53.2  \\ 
 % \hline
 \bottomrule
\end{tabular}
% \vspace{-0.25cm}
\caption{The performance of LBP under different $n_a$ on OV-COCO.}
% \vspace{-0.25cm}
\label{tab:ablation_na}
\end{table}


\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l|ccc}
% \hline
\toprule
$\gamma$  &   $\textrm{AP}^n_{50}$ & $\textrm{AP}^b_{50}$ & $\textrm{AP}_{50}$   \\ 
% \hline
\midrule
$0.01$ & 37.6 & 58.8 & 53.2  \\ 
$0.02$ & 37.8 & 58.7 & 53.2\\ 
$0.05$ & 37.5  & 58.7  & 53.2  \\ 
 % \hline
 \bottomrule
\end{tabular}
% \vspace{-0.25cm}
\caption{The performance of LBP under different $\gamma$ on OV-COCO.}
% \vspace{-0.25cm}
\label{tab:ablation_gamma}
\end{table}

\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l|ccc}
% \hline
\toprule
$\lambda_{bg}$  &   $\textrm{AP}^n_{50}$ & $\textrm{AP}^b_{50}$ & $\textrm{AP}_{50}$   \\ 
% \hline
\midrule
$0.01$ & 37.4 & 58.9 & 53.3  \\ 
$0.05$ & 37.8 & 58.7 & 53.2\\ 
$0.1$ &  37.8 &  58.6  & 53.1 \\ 
 % \hline
 \bottomrule
\end{tabular}
% \vspace{-0.25cm}
\caption{The performance of LBP under different $\lambda_{bg}$ on OV-COCO.}
% \vspace{-0.25cm}
\label{tab:ablation_lambda}
\end{table}

==> tables/Ablation_pr.tex <==
\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{l|ccc}
% \hline
\toprule
Method  &   $\textrm{AP}^n_{50}$ & $\textrm{AP}^b_{50}$ & $\textrm{AP}_{50}$   \\ 
% \hline
\midrule
LBP w/o IPR & 35.6 & 58.7 &  52.7 \\
LBP w/o $\tilde{\mathbf{\Sigma}}^{o}$ & 35.5 & 57.8 & 52.0 \\ 
 LBP (ours) &  37.8 &  58.7   &  53.2    \\ 
 % \hline
 \bottomrule
\end{tabular}
% \vspace{-0.25cm}
\caption{Additional ablation study results of IPR on OV-COCO.
}
% \vspace{-0.50cm}
\label{tab:ablation_pr}
\end{table}
